Some IHX type relations on trivalent graphs and symplectic representation theory

We consider several algebras that arise in the study of the mapping class group (by means of topology and Hodge theory) and describe their symplectic-invariant parts in terms of algebras on trivalent graphs.

==> draws/SymIHX.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(5104,939)(0,-10)
\thicklines
\path(12,912)(912,912)
\path(12,12)(912,12)
\path(1812,912)(1812,12)
\path(2712,912)(2712,12)
\path(3612,912)(4512,12)
\path(3612,12)(3987,387)
\path(4137,537)(4512,912)
\path(1812,462)(2712,462)
\path(3837,237)(4287,237)
\path(462,912)(462,12)
\put(1212,387){\makebox(0,0)[lb]{$+$}}
\put(3012,387){\makebox(0,0)[lb]{$+$}}
\put(4812,387){\makebox(0,0)[lb]{$=0$}}
\end{picture}


==> draws/circle.tex <==
\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(1811,1632)(0,-10)
\thicklines
\put(825.000,1158.000){\arc{900.000}{1.5708}{4.7124}}
\path(945.000,1638.000)(825.000,1608.000)(945.000,1578.000)
\put(825.000,1158.000){\arc{900.000}{4.7124}{7.8540}}
\path(375,408)(1275,408)
\path(825,708)(825,408)
\path(795.000,528.000)(825.000,408.000)(855.000,528.000)
\put(750,933){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{rm}\$1\$}}}}}
\put(0,108){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{rm}\$x\_2\$}}}}}
\put(1350,108){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{rm}\$x\_1\$}}}}}
\put(675,33){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{rm}\$2\$}}}}}
\end{picture}


==> draws/enn.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(3334,1774)(0,-10)
\thicklines
\put(2965.864,688.591){\arc{716.720}{5.5921}{7.2581}}
\put(1806.773,2215.864){\arc{4370.716}{1.2155}{2.3209}}
\put(317,917){\ellipse{618}{618}}
\put(1142,1442){\ellipse{618}{618}}
\put(2117,1442){\ellipse{618}{618}}
\put(3017,1142){\ellipse{618}{618}}
\put(2867,317){\ellipse{618}{618}}
\path(542,1142)(842,1292)
\path(1442,1442)(1817,1442)
\path(2417,1367)(2717,1292)
\put(1217,242){\makebox(0,0)[lb]{$\ldots$}}
\end{picture}


==> draws/equivIH.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(10369,944)(0,-10)
\thicklines
\put(465.357,464.000){\arc{910.714}{1.4173}{4.8659}}
\path(535,914)(1435,914)
\path(535,14)(1435,14)
\path(985,914)(985,14)
\path(2935,914)(2935,14)
\path(3835,914)(3835,14)
\path(2935,464)(3835,464)
\put(2865.357,464.000){\arc{910.714}{1.4173}{4.8659}}
\put(1735,389){\makebox(0,0)[lb]{$=$}}
\path(8935,914)(8935,14)
\path(9835,914)(9835,14)
\path(8935,464)(9835,464)
\put(5865.357,464.000){\arc{910.714}{1.4173}{4.8659}}
\put(6905.000,464.000){\arc{910.824}{4.5581}{8.0083}}
\put(8865.357,464.000){\arc{910.714}{1.4173}{4.8659}}
\put(9905.000,464.000){\arc{910.824}{4.5581}{8.0083}}
\path(5935,914)(6835,914)
\path(5935,14)(6835,14)
\path(6385,914)(6385,14)
\put(7735,389){\makebox(0,0)[lb]{$=$}}
\end{picture}


==> draws/rIH.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(7896,941)(0,-10)
\thicklines
\put(4212,463){\ellipse{450}{450}}
\put(6762,463){\ellipse{912}{912}}
\path(12,913)(912,913)
\path(12,13)(912,13)
\path(1812,913)(1812,13)
\path(2712,913)(2712,13)
\path(1812,463)(2712,463)
\path(462,913)(462,13)
\path(4212,913)(4212,688)
\path(4212,238)(4212,13)
\path(6762,913)(6762,13)
\put(1137,388){\makebox(0,0)[lb]{$=$}}
\put(4737,388){\makebox(0,0)[lb]{$=0$}}
\put(7512,388){\makebox(0,0)[lb]{$=0$}}
\end{picture}


==> draws/theta.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(2676,1834)(0,-10)
\thicklines
\put(1282.500,916.500){\arc{1785.063}{4.7040}{6.2916}}
\put(1282.500,901.500){\arc{1785.063}{6.2748}{7.8624}}
\path(1154.752,1780.009)(1275.000,1809.000)(1155.256,1840.007)
\put(1267.500,916.500){\arc{1785.063}{3.1332}{4.7208}}
\path(1155.256,-22.007)(1275.000,9.000)(1154.752,37.991)
\put(1267.500,901.500){\arc{1785.063}{1.5624}{3.1500}}
\path(129.000,912.000)(225.000,834.000)(177.000,948.000)
\put(375.000,946.500){\arc{375.000}{2.4981}{6.9267}}
\path(2373.000,948.000)(2325.000,834.000)(2421.000,912.000)
\put(2175.000,946.500){\arc{375.000}{2.4981}{6.9267}}
\path(375,909)(1275,909)
\path(1395.000,939.000)(1275.000,909.000)(1395.000,879.000)
\path(1275,909)(2175,909)
\put(0,534){\makebox(0,0)[lb]{$1$}}
\put(2400,534){\makebox(0,0)[lb]{$2$}}
\end{picture}


==> draws/x2y.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(1834,408)(0,-10)
\thicklines
\path(150,12)(1350,12)
\path(1230.000,-18.000)(1350.000,12.000)(1230.000,42.000)
\put(0,237){\makebox(0,0)[lb]{$x_{a}$}}
\put(1050,237){\makebox(0,0)[lb]{$y_{a}$}}
\end{picture}


==> draws/y2x.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(1834,408)(0,-10)
\thicklines
\path(150,12)(1350,12)
\path(1230.000,-18.000)(1350.000,12.000)(1230.000,42.000)
\put(1050,237){\makebox(0,0)[lb]{$x_{a}$}}
\put(0,237){\makebox(0,0)[lb]{$-y_{a}$}}
\end{picture}

